Narrative Flattening: How Post-Training Compresses Thematic, Affective, and Stylistic Variation in LLM Fiction

Large language models produce fluent fiction, yet their creative output is widely seen as flat. We ask where this quality originates in the training and whether it affects different domains of human fiction equally. We construct a matched story-continuation paradigm across StoryStar (public-platform), TMAS (prompt-guided), and The New Yorker (professional literary)-and compare continuations from four OLMo 32B checkpoints (Base, SFT, DPO, RLVR) against matched human text. Because these checkpoints share architecture, scale, tokenizer, and pretraining, the design isolates the post-training effect. We measure each continuation along three sentence-level dimensions: thematic motion, affective prevalence, and linguistic diversity. Across all three, post-training compresses dynamic variation: thematic transitions become more uniform, high-intensity emotions give way to neutrality, and stylistic diversity across stories shrinks. We term this progressive loss narrative flattening. The effect is directionally stable across story domains but gap size depends on the human baseline: professional literary fiction is compressed most, while public-platform and prompt-guided stories show smaller gaps, consistent with their human baselines sitting closer to the model's default rhythm. Post-trained endpoints converge across domains, suggesting alignment produces a continuation regime largely insensitive to the source domain's narrative texture.

==> Sections/06-DiscussionOLD.tex <==
\section{Discussion}
\label{sec:discussion}

\paragraph{Post-training as narrative regularization.}
Our results suggest that post-training acts as a form of narrative regularization. 
The base model is not simply human-like: in affective space, it can be over-marked, and in stylistic space, it spreads across a broad and unstable region. 
Supervised fine-tuning, preference optimization, and reinforcement learning make generation more controlled and conventionally well-formed, but this control is achieved by suppressing variation. Thematic jumps become more uniformly sized, affective pressure is muted, and linguistic habits collapse into a narrower attractor. 
This helps explain why aligned fiction can be fluent and readable while still feeling mechanical: the issue is not sentence-level grammaticality, but the loss of dynamic contrast across a continuation.

\paragraph{Flattening is relative to heterogeneous human baselines.}
A central implication of our cross-domain design is that there is no single human baseline for creative writing. Professional literary fiction, prompt-guided fiction, and public-platform fiction differ before any model is introduced. 
They vary in affective charge, stylistic signature, and the rhythm with which they move through narrative space. Evaluating model fiction against a pooled human reference would blur these differences. Domain-sensitive evaluation reveals a sharper pattern: post-training pulls different source domains toward similar endpoints, even when the human continuations they replace begin from different narrative regimes.

\paragraph{Why professional fiction is compressed most.}
The largest distortion appears for professional literary fiction because its human baseline lies farthest from the post-trained model's continuation regime.
\textit{The New Yorker} continuations carry higher affective charge, lower neutrality, and a distinctive stylistic distribution; post-trained models move away from this profile and toward a region closer to common-fiction baselines.
The smaller gaps for \textsc{StoryStar} and \textsc{Tell Me A Story} therefore should not be interpreted as evidence that the model writes these domains better. Rather, these domains already sit closer to the regime that post-training favors. We also do not claim to observe the causal role of the
training data directly. 
Without access to the full pretraining and post-training mixtures, the safest conclusion is geometric: the post-trained endpoint lies closer to common-fiction baselines than to professional literary fiction.

\paragraph{Implications for creative-writing assistants.}
These findings complicate the usual success criteria for post-training. 
In many assistant tasks, reduced variation is desirable: users often want consistent, clear, and predictable answers. In fiction, however, variation is part of the task. 
Thematic unevenness, affective volatility, and stylistic breadth are not noise to be removed; they are part of how stories produce literary texture.
Creative-writing assistants may therefore require different alignment targets from general-purpose assistants. 
Rather than rewarding only coherence, helpfulness, and surface-level readability, future systems may need objectives that preserve the narrative texture of the source domain being continued.

\paragraph{Toward evaluations of creative diversity.}
Our results also suggest that human preference alone is an incomplete evaluation target for creative writing. A continuation may be readable, coherent, and even preferred in isolation while still making a collection of stories more homogeneous. 
Narrative flattening metrics provide a complementary diagnostic:
they ask whether models preserve the variance structure of human fiction, not only whether they produce plausible prose. 
This distinction is especially important for co-writing systems, where the cultural cost may not be one bad story, but the gradual convergence of many stories toward the same rhythm, affect, and voice.

==> manifold_precision.tex <==
\paragraph{In-human-manifold precision.}
We estimate a human linguistic-habit manifold from human sentence embeddings. 
Embeddings are standardized using human mean and variance, reduced with PCA, 
and assigned an inclusion radius $\epsilon$ equal to the 95th percentile of 
human 5-nearest-neighbor distances. 
For model sentence embedding $m_j$, let 
$d(m_j,H)$ be its nearest-neighbor distance to the human set. 
Precision is
\[
    \mathrm{Prec}(M)
    =
    \frac{1}{|M|}
    \sum_{m_j \in M}
    \mathbbm{1}\left[d(m_j,H) \leq \epsilon\right].
\]
High precision with low across-story variance indicates that model writing lies 
inside a human-like region but occupies it narrowly.

